Declarative Programming for Microcontrollers -- Datalog on Arduino

In this paper we describe an approach to programming microcontrollers based on the Arduino platform using Datalog as a clear and concise description language for system behaviors. The application areas of cheap and easily programmable microcontrollers, like robotics, home automation, and IoT devices hold mainstream appeal and are often used as motivation in natural science and technology teaching. The choice of programming languages for microcontrollers is severely limited, especially with regard to rule-based declarative languages. We use an approach that is based on the Dedalus language augmented with operations that allow for side-effects and takes the limited resources of a microcontroller into account. Our compiler and runtime environment allow to run Datalog programs on Arduino-based systems.

==> makefile <==
#==============================================================================
# Project:	Some Progress on Benchmarks of Deductive and Relational DBs
# Version:	In Preparation (for WLP 2018)
# Module:	makefile
# Purpose:	Definitions for Project Management using "make"
# Last Change:	11.06.2018
# Language:	make
# Authors:	Stefan Brass
# Email:	brass@informatik.uni-halle.de
# Address:	University of Halle, Von-Seckendorff-Platz 1, D-06120 Halle
# Copyright:	(c) 2000-2018 by Stefan Brass
# Copying:	Please ask for permission before doing that.
#==============================================================================

#------------------------------------------------------------------------------
# This makefile knows about the following goals:
# ==============================================
# make:		runs pdfLaTeX to generate pdf file
#		Note: The dependency from the .aux-files is ignored,
#		so used "make again" to force the execution of TeX.
# make again:	run pdfLaTeX to generate the .pdf-file in any case.
# make dvi:	run standard LaTeX to generate dvi file
# make view:	run evince to have a preview.
#		pdfLaTeX is called first, if necessary.
# make dv:	Use xdvi for preview. Standard LaTeX is run first if necessary.
# make prt:	prints the input.
# make sub:	prints a subrange of the input.
#		The first and the last page are queried interactively.
# make clean:	removes temporary files.
# make bib:	generates bibliography (.bbl-file) via BibTeX.
# make bbl:	equivalent to "make bib".
# make ind:	generates an index via makeindex.
# make shar:	generates a shell archive from the tex input files,
#		the makefile and OTHER files.
#------------------------------------------------------------------------------

# The main file, without the extension ".tex":
FILE	= wlp19# Don't leave any spaces after the filename !!!

# The Include files (except those in TMPINCL) the document depends on:
INCLUDE	= c1_intro.tex \
	c3_dedalus_ext.tex \
	c2_target_hardware.tex \
	c4_evaluation.tex \
	c5_iolit.tex \
	c6_rte.tex \
	c7_macros.tex \
	c8_conclusion.tex

# Temporary TeX files. Be careful, these are deleted with "make clean"!
TMPINCL =

# Other files, which should be put into the archive:
OTHER	= $(FILE).aux $(FILE).bbl

# The name of the printer is constantly changing:
PRINTER	= alpha

# Which version of LaTeX:
LATEX	= latex
PDFLATEX= pdflatex

# Default goal:
all: $(FILE).pdf
#all: $(FILE).dvi
#all: $(FILE).ps

#==============================================================================
# Run TeX:
#==============================================================================

$(FILE).dvi: $(FILE).tex $(INCLUDE)
	$(LATEX) $(FILE).tex

dvi: $(FILE).tex $(INCLUDE)
	$(LATEX) $(FILE).tex

$(FILE).pdf: $(FILE).tex $(INCLUDE)
	$(PDFLATEX) $(FILE).tex

pdf: $(FILE).tex $(INCLUDE)
	$(PDFLATEX) $(FILE).tex

again: pdf


#==============================================================================
# Print DVI-File:
#==============================================================================

prt: $(FILE).dvi
	dvips -P$(PRINTER) $(FILE).dvi

#==============================================================================
# Print Subrange of DVI-File:
#==============================================================================

DVOSUB	= \
  dvips -P$(PRINTER) -p $$f -n `expr $$l - $$f + 1` $(FILE).dvi

sub: $(FILE).dvi
	@echo -n 'Enter first page to print: '; \
	read f; \
	echo -n 'Enter last page to print: '; \
	read l; \
	echo "$(DVOSUB)"; \
	$(DVOSUB)

#==============================================================================
# Preview DVI-File:
#==============================================================================

view: pv

pv: $(FILE).pdf
	evince $(FILE).pdf

dv: $(FILE).dvi
	xdvi -geometry +810+34 -s 8 -S 20  -paper a4 $(FILE).dvi

dv2: $(FILE).dvi
	xdvi -geometry +360+50 -expert -s 8 -S 20  -bg white $(FILE).dvi

gv: $(FILE).ps
	ghostview -bg white $(FILE).ps

#==============================================================================
# Create Postscript File:
#==============================================================================

ps: $(FILE).ps

$(FILE).ps: $(FILE).dvi
	dvips -P$(PRINTER) -o $(FILE).ps $(FILE).dvi

half: $(FILE)_2.ps

$(FILE)_2.ps: $(FILE).ps
	psnup -2 $(FILE).ps > $(FILE)_2.ps

quad: $(FILE)_4.ps

$(FILE)_4.ps: $(FILE).ps
	psnup -4 -m10 $(FILE).ps > $(FILE)_4.ps

#==============================================================================
# Create index:
#==============================================================================

ind: $(FILE).ind

$(FILE).ind: $(FILE).idx
	makeindex -s ../makeind.sty -g $(FILE).idx

#==============================================================================
# Create bibliography:
#==============================================================================

bib: $(FILE).bib

$(FILE).bib: $(FILE).aux
	bibtex $(FILE)

#==============================================================================
# Remove temporal files:
#==============================================================================

clean:
	rm -f *.log
	rm -f *.dvi
	rm -f *.aux
	rm -f *.tmp
	rm -f *.out

very_clean: clean
	rm -f $(FILE).ps
	rm -f $(FILE)_2.ps
	rm -f $(FILE)_4.ps

#==============================================================================
# Generate shell archive (optionally compressed):
#==============================================================================

$(FILE).shar: $(FILE).tex $(INCLUDE) makefile $(OTHER)
	shar >$(FILE).shar $(FILE).tex $(INCLUDE) makefile $(OTHER)

$(FILE).comp_shar: $(FILE).tex $(INCLUDE) makefile $(OTHER)
	shar >$(FILE).shar $(FILE).tex $(INCLUDE) makefile $(OTHER)
	compress $(FILE).shar
	uuencode $(FILE).shar.Z $(FILE).shar.Z >$(FILE).shar.Z.uu
	rm $(FILE).shar.Z

#==============================================================================
# Implicit Rules, Generate all Slides:
#==============================================================================

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex $(SUFFIXES)

.tex.dvi: $(INCLUDE)
	$(LATEX) $(FILE).tex

.dvi.ps:
	dvips -P$(PRINTER) -o $*.ps $(FILE).dvi

